Dis-S2V: Discourse Informed Sen2Vec

Vector representation of sentences is important for many text processing tasks that involve clustering, classifying, or ranking sentences. Recently, distributed representation of sentences learned by neural models from unlabeled data has been shown to outperform the traditional bag-of-words representation. However, most of these learning methods consider only the content of a sentence and disregard the relations among sentences in a discourse by and large. In this paper, we propose a series of novel models for learning latent representations of sentences (Sen2Vec) that consider the content of a sentence as well as inter-sentence relations. We first represent the inter-sentence relations with a language network and then use the network to induce contextual information into the content-based Sen2Vec models. Two different approaches are introduced to exploit the information in the network. Our first approach retrofits (already trained) Sen2Vec vectors with respect to the network in two different ways: (1) using the adjacency relations of a node, and (2) using a stochastic sampling method which is more flexible in sampling neighbors of a node. The second approach uses a regularizer to encode the information in the network into the existing Sen2Vec model. Experimental results show that our proposed models outperform existing methods in three fundamental information system tasks demonstrating the effectiveness of our approach. The models leverage the computational power of multi-core CPUs to achieve fine-grained computational efficiency. We make our code publicly available upon acceptance.

==> ack.tex <==
%This section is optional; it is a location for you
%to acknowledge grants, funding, editing assistance and
%what have you.  In the present case, for example, the
%authors would like to thank Gerald Murray of ACM for
%his help in codifying this \textit{Author's Guide}
%and the \textbf{.cls} and \textbf{.tex} files that it describes.


==> app.tex <==
%Appendix A

\newpage

\section{Noise Contrastive Estimation}

We can train our models by maximizing the log likelihood (or minimizing cross entropy) of the data using gradient-based online methods, such as stochastic gradient descent with the \emph{backpropagation} algorithm. Unfortunately, training could be impractically slow because for each training instance the softmax function in the output layer needs to compute a summation over all nodes in the graph. Noise contrastive estimation or NCE \cite{Gutmann.Hyvarinen:10,Mnih.Teh:12} provides an efficient and stable way to avoid this repetitive computation.  

We can re-write the softmax in Equation \ref{eq:n2v} as follows:

\begin{eqnarray}
P(n_i|u, \phi) &=& \frac{\exp(\omega(n_i)^T \phi(u))}{\sum_{v \in V} \exp(\omega(v)^T \phi(u))} \nonumber \\
			   &=& \frac{\exp(\omega(n_i)^T \phi(u))}{Z(\phi(u), v, \omega)} \label{soft_unnor}
\end{eqnarray}


\noindent where $Z(.)$ is the normalization factor, which is considered as an additional parameter along with the regular parameters $\phi$ and $\omega$. It has been found that fixing $Z(.)$ to $1$ instead of learning it in training does not affect the model performance \cite{Mnih.Teh:12}. Hence, we set $Z(.)$ to $1$ during training the model.


In training with NCE, for each training instance $(u, n_i)$, we add $M$ noise samples $\{(u, n_i^m)\}_{m=1}^{M}$ by sampling $n_i^m$ from a known noise distribution $\psi$ (e.g., \texttt{unigram, uniform}); NCE loss is then defined as such to discriminate a \emph{true} instance from a \emph{noisy} one. Let $C$ $\in$ $\{0,1\}$ denote the class of an instance with $C$ $=$ $1$ indicating \emph{true} and $C$ $=$ $0$ indicating \emph{noise}. NCE maximizes the following objective:

%see the plate notation in Figure \ref{fig:NNJM_NCE}. 
\begin{align}
J(\phi)  &=  \log P(C = 1|n_i,\phi(u), \omega) + \sum_{m=1}^{M} \log P(C = 0|n_i^m, \phi(u), \psi)  \nonumber  \\
         &=  \log \left[ P(n_i|C=1,\phi(u),\omega) P(C = 1|\pi) \right] +  \nonumber \\
         & \hspace{1cm} \sum_{m=1}^{M}  \log [P(n_i^m|C=0,u,\psi) P(C = 0|\pi)] \label{eq:nce-cost-tmp}
\end{align}

After removing the constant terms (class conditionals and denominators), the above equation can be simplified as:

%\noindent where $Q = P(y_n, C=1|\mathbf{x}_n,\theta,\pi) + P(y_n^m, C=0|\mathbf{x}_n,\psi,\pi)$ is a normalization constant. After removing the constant terms, Equation \ref{nce-cost} can be simplified as:


\begin{align}
J(\phi)  &= \omega(n_i)^T \phi(u) + \sum_{m=1}^{M} \log P(n_i^m|u,\psi)  \label{eq:nce-cost} 
\end{align}


\noindent where $\psi$ is the noise distribution. NCE reduces the number of computations needed at the output layer from $|V|$ to $M+1$, where $M$ is a small number compared to $|V|$. 

%In all our experiments we use NCE loss with $M$ $=$ $100$ samples in accordance to \cite{Mnih.Teh:12}.

\subsection{Negative Sampling}

It has been shown that NCE approximately maximizes softmax probability \cite{Mnih.Teh:12}. In our representation methods, we are concerned with learning high-quality vector representations, so we are free to
simplify NCE as long as the quality of the representations are retained. We change the NCE objective in Equation \ref{eq:nce-cost} as follows: 

\begin{align}
J(\phi)  &= \log \sigma(\omega(n_i)^T \phi(u)) + \sum_{m=1}^{M} \mathbb{E} \left[ \log \sigma (- \omega(n_i^m)^T \phi(u)) \right]  \label{eq:neg-cost} 
\end{align}

\noindent where $\sigma()$ is the sigmoid function. Thus the loss function in Equation \ref{eq:neg-cost} mimics the loss of logistic regression to distinguish the target node $n_i$ from the noise samples $n_i^m$. This method is called negative sampling. The main difference between the Negative sampling and NCE is that NCE needs both samples and the probabilities from the noise distribution $\psi$, while Negative sampling uses only
samples. 

%And while NCE approximately maximizes the log probability of the softmax, this property
%is not important for our application.















==> regularized-sen2vec-bak.tex <==
% !TEX root = sen2vec-www-17.tex
%%%
%%% Regularized Sen2Vec models
%%%


Rather than retrofitting the vectors from the content-based model on the discourse graph as a post-processing step, we can incorporate the neighborhood information directly into the objective function of the content-based model as a regularizer, and learn the Dis-S2V vectors in a single step. We define the following objective to minimize:      

\begin{equation}
J(\phi) = \sum_{\mathbf{v} \in V} \Big[ L(\mathbf{v}) + \hspace{-0mm} \lambda \hspace{-0.2cm} \sum_{(u,v)\in E} \hspace{-0.5mm}  W_{u,v} ||\phi(\mathbf{u}) - \phi(\mathbf{v})||^2 \Big] \label{eq:reg}
\end{equation} 

\noindent where the first component $L(\mathbf{v})$ refers to the negative log likelihood loss of the content based model described in Section \ref{sec:sen2vec}, i.e., Equation \ref{eq:dm} for DM and Equation \ref{eq:dbow} for DBOW. The second component is the graph smoothing regularizer with $\lambda$ being the regularization strength. Since this model learns the vectors from scratch in one shot by considering information from both sources, the two components can be better adjusted to produce better quality vectors.  


\subsubsection{Possible Extensions}


Notice that the regularizer in Equation \ref{eq:reg} considers only first-order neighborhood. One possible extension would be to consider the neighborhood sampled by the stochastic sampling method of Node2Vec, which is more flexible. Another interesting extension of the model would be, rather than defining the regularizer as a weighted distance between two vectors, we can use the objective of Node2Vec as the regularizer and minimize the combined negative log likelihood. More formally, we can redefine the model in Equation \ref{eq:reg} as:     

\begin{equation}
J(\phi) = \sum_{\mathbf{v} \in V} \Big[ L(\mathbf{v}) - \hspace{-0mm} \lambda \hspace{-0.2cm} \sum_{\mathbf{n}_i \in N(\mathbf{v})} \log P(\mathbf{n}_i|\phi(\mathbf{v})) \Big] \label{eq:reg_n2v}
\end{equation} 
 
The first component minimizes the cross entropy with respect to what \emph{words} are observed in a sentence, while the second component minimizes the cross entropy with respect to what \emph{sentences} are observed in the neighborhood of the sentence. Although these extensions are interesting, they are left in this paper as future work.





==> word-semantics.tex <==

The Dis-S2V models described so far trains the vectors by exploiting the content of a sentence and its neighborhood in the discourse graph. Notice that the DM model in Figure \ref{s2v} (a) also trains word representation as a byproduct. Recent work has shown that lexical semantic relations (e.g., synonymy, hypernymy) encoded in semantic lexicons (e.g., WordNet \cite{Miller:95}, Framenet \cite{Baker:98}) can improve the quality of word vectors that are trained solely on the sentence contents \cite{Xu:2014,faruqui:2015:Retro,yu:dredze:2014}. Therefore, in addition to the discourse graph, semantic lexicons can be used as a word-level information source to refine the word vectors, which should in turn refine the sentence vectors. Following previous work, we convert any kind of lexicon into a network, where semantically similar words defined by the lexicon become neighbors in the graph and then induce this information as another word-level graph smoothing factor.                



